A Resolution of the Diagonal for Toric Deligne-Mumford Stacks

Beilinson's resolution of the diagonal for complex projective space was generalized by Bayer-Popescu-Sturmfels for any unimodular toric variety. Here, we give a resolution of the diagonal for any smooth toric variety (viewed as a toric Deligne-Mumford stack) in families by deformation of the cellular complex of Bayer-Popescu-Sturmfels and show that the cokernel of this resolution gives the diagonal, modulo torsion from the irrelevant ideal. Furthermore, we give a resolution of the diagonal for a toric Deligne-Mumford stack associated to the global quotient of a smooth toric variety by a finite abelian group.

==> abstract.tex <==
% +--------------------------------------------------------------------+
% | Abstract Page
% +--------------------------------------------------------------------+

\pagestyle{empty}
%\vspace{1cm}
\setlength{\baselineskip}{0.8cm}

%\indent

% +--------------------------------------------------------------------+
% | Enter the text of your abstract below.  The abstract should does not have an upper word limit.  
% +--------------------------------------------------------------------+

Beilinson's resolution of the diagonal for complex projective spaces gives a locally free resolution of the structure sheaf of the diagonal as a Koszul complex, which gives a Fourier-Mukai transform inducing the identity on objects in the derived category of coherent sheaves of $\mathbb{P}^n$. Since $\mathbb{P}^n$ is a toric variety, we can ask for a resolution of the diagonal of an arbitrary toric variety. While resolutions of the diagonal are known for toric varieties which are unimodular in the sense of Bayer-Popescu-Sturmfels, in order to generalize a resolution of the diagonal for simplicial toric varieties, we must consider smooth Deligne-Mumford toric stacks associated to a given simplicial toric variety. Here, the diagonal can fail to be a closed substack because of non-zero stabilizers at the origin, so that a direct generalization of Beilinson's resolution will not work. For a simplicial toric variety $X_\Sigma' = \faktor{X_\Sigma}{\mu}$ which is a global quotient  of a toric variety $X_\Sigma$ which is unimodular in the sense of Bayer-Popescu-Sturmfels by the finite abelian group $\mu$, let $\tilde{L}$ denote the lattice of principal divisors of $X_\Sigma'$. Up to isomorphism, we can choose $L$, the lattice of principal divisors of $X_\Sigma$ such that $\tilde{L}\subset L$ is cofinite, $L$ is a unimodular lattice in the sense of Bayer-Popescu-Sturmfels, and $\faktor{L}{\tilde{L}}\cong \mu$. Here, we construct a diagonal object inducing the kernel of a Fourier-Mukai transform by adapting a known resolution of the diagonal for $X_\Sigma'$ unimodular due to Bayer-Popescu-Sturmfels. Furthermore, we strengthen this result to give a resolution of the diagonal for global quotients $X_\Sigma' = \faktor{X_\Sigma}{\mu}$ for $X_\Sigma$ a smooth toric variety by the finite abelian group $\mu$ by showing that the cokernel of an inclusion $coker(M_{\Lambda(L)} \hookrightarrow Im(f))$ from an associated map $f$ is zero, so that the complex $\mathcal{F}_{H^\epsilon_L/\tilde{L}}^\bullet$ gives a resolution of the diagonal $\mathcal{O}_\Delta$, modulo torsion from the irrelevant ideal $I_{irr}$ for the product $X_\Sigma \times X_\Sigma$. This also strengthens the construction of the diagonal object giving the kernel of a Fourier-Mukai transform inducing the identity in $D^b_{Coh}(X_\Sigma')$ to $X_\Sigma'$ a global quotient of a smooth toric variety by a finite abelian group. 






%For toric varieties which are unimodular in the sense of Cox-Little-Schenck, we construct a ``deformed resolution." ... For simplicial toric varieties whose associated toric DM-stack $\mathcal{X}$ admits a finite, dominant map $\faktor{X_\Sigma'}{G}$ as above, we can ask whether a resolution of the diagonal for $\mathcal{X}$ is present inside $D^b(\faktor{X_\Sigma'})$ via pullback. 







 

%Enter the text of your abstract in the abstract.tex file. There is not a size limit for this section. Be sure to delete the text below before you submit your ETDR.

%This template uses a separate file for each section of your ETDR:  title page, abstract, preface, chapters, reference, etc.  This makes it easier to organize and work with a lengthy document.  The template is configured with page margins required by the Graduate School and will automatically create a table of contents, lists of tables and figures, and PDF bookmarks.

%The file etdrtemplate.tex is the "master" file for the ETDR template.  This is the file you need to process with PDFLaTeX in order to produce a PDF version of your ETDR.  See the comments in the etdrtemplate.tex and other files for details on using the template.  You are not required to use the template, but it can save time and effort in making sure your ETDR meets the Graduate School formatting requirements.

%Although the template gives you a foundation for creating your ETDR, you will need a working knowledge of LaTeX in order to produce a final document.  You should be familiar with LaTeX commands for formatting text, equations, tables, and other elements you will need to include in your ETDR.


==> abstracttitle.tex <==
% +--------------------------------------------------------------------+
% | Abstract Title Page
% |
% |This page is required only for doctoral dissertations.
% +--------------------------------------------------------------------+

% +--------------------------------------------------------------------+
% | This page should not contain a page number.  We use the
% | \thispagestyle[empty] command below to suppress page numbers
% | and other style elements.
% +--------------------------------------------------------------------+

\thispagestyle{empty}

% +--------------------------------------------------------------------+
% | The Abstract Title page begins here
% +--------------------------------------------------------------------+

\pdfbookmark[0]{Title Page}{PDFTitlePage}
%\setcounter{page}{1}

\begin{center}

   \vspace{1cm}

% +--------------------------------------------------------------------+
% | Enter the title of your ETDR below.  For 2017 and on, use "Sentence case" (not ALL CAPS).
% | For details, see:  k-state.edu/grad/etdr/create/sentencecase.html 
% +--------------------------------------------------------------------+

   \large A Resolution of the Diagonal for Some Toric D-M Stacks \\

   \vspace{0.5cm}

   by\\

   \vspace{0.5cm}

% +--------------------------------------------------------------------+
% | Enter your name below in standard name format (not ALL CAPS).
% +--------------------------------------------------------------------+

   \large Reginald Cyril Wallis Anderson\\

   \vspace{0.5cm}

% +--------------------------------------------------------------------+
% | On the line below, replace "Enter Your Previous Degrees"
% | with your previous degrees in mixed case. Include the abbreviation
% | for the degree, the name of the university, and the year separated
% | by commas. For example:
% |
% |    B.A., University of Illinois, 2000
% |
% | If desired, it is acceptable to include a city or country with
% | the university name. For example:
% |
% |    B.S., Jillian University, China, 2002
% |
% | Each degree should appear on a separate line.  Use the \\
% | command to create a line break.
% +--------------------------------------------------------------------+

   B.A., Colorado College, 2013\\
   M.S., Kansas State University, 2019\\

   \vspace{0.55cm}
   \rule{2in}{0.5pt}\\
   \vspace{0.75cm}

   {\large AN ABSTRACT OF A DISSERTATION}\\

   \vspace{0.5cm}
   \begin{singlespace}
   submitted in partial fulfillment of the\\
   requirements for the degree\\
   \end{singlespace}

   \vspace{0.5cm}

% +--------------------------------------------------------------------+
% | On the line below, enter the name of your earned degree in ALL
% | CAPITAL LETTERS.  For example: DOCTOR OF PHILOSOPHY
% +--------------------------------------------------------------------+


   {\large DOCTOR OF PHILOSOPHY}\\
   \vspace{0.5cm}

% +--------------------------------------------------------------------+
% | On the two lines below, enter the name of your department and the
% | name of the college in mixed case.  For example:
% |
% |     Biochemistry Department
% |     College of Arts and Sciences
% +--------------------------------------------------------------------+

   \begin{singlespace}
   Mathematics Department\\
  College of Arts and Sciences\\
   \end{singlespace}

   \vspace{0.5cm}

   \begin{singlespace}
   {\Large KANSAS STATE UNIVERSITY}\\
   Manhattan, Kansas\\
   \end{singlespace}

% +--------------------------------------------------------------------+
% | On the line below, replace "Graduation Year" with the four-digit year
% | of your graduation. For example:
% |
% |     2017
% +--------------------------------------------------------------------+

   2023\\
   \vspace{1cm}

\end{center}


==> chapter4.tex <==


% +--------------------------------------------------------------------+
% | Sample Chapter 4
% +--------------------------------------------------------------------+

\cleardoublepage

% +--------------------------------------------------------------------+
% | Replace "This is Chapter 3" below with the title of your chapter.
% | LaTeX will automatically number the chapters.                      
% +--------------------------------------------------------------------+

\appendix
\chapter{Appendix}
\textbf{Lemma 2 from Section~\ref{lemmata} for $X_\Sigma$ smooth, Fano, not necessarily unimodular}: For any $p \in \mathcal{H}_L^\epsilon(0)$ and $\sigma \in \Sigma(n)$, there exists $v_\sigma \in L$ with $(p+v_\sigma)_\rho <0$ only on $\sigma(1)$, and $(p+v_\sigma)_\rho >0$ for $\rho\not\in\sigma(1)$.  

\begin{proof} We previously noted that since $X_\Sigma$ is Fano, there exists $v\in L$ such that

\[ \begin{cases} v(u_\rho)<0 & \forall \text{ }\rho\in\sigma(1),\\ v(u_{\rho'}) \geq 0 & \forall \rho' \not\in\sigma(1) \end{cases} \] 

Now there exists $r\in \Z$ such that $(r\cdot v)_\rho <<0$ for all coordinates with $\rho\in\sigma(1)$ so that all $\rho\in \sigma(1)$ become much less than any coordinate $\rho'\not\in\sigma(1)$. Additionally, there exists a unique $\tilde{v}\in L$ such that \[ \begin{cases}  (p+\tilde{v})(u_\rho)= 0 & \forall\text{ }\rho\in\sigma(1)\\ (p+\tilde{v})(u_{\rho'}) > 0 & \forall\text{ }\rho'\not\in \sigma(1). \end{cases} \]

Now adding on sufficiently large multiples of $v$ and $\tilde{v}$ ensure that there exists $r, k\in \Z$ such that $v_\sigma = rv + k\tilde{v}$ gives that $p+v_\sigma$ satisfies

\[ \begin{cases} (p + v_\sigma)_\rho < 0 & \text{ iff } \rho\in\sigma(1),\\ (p+v_\sigma)_\rho  >0 & \text{ otherwise}. \end{cases} \] \end{proof}

==> chapter5.tex <==
% +--------------------------------------------------------------------+
% | Sample Chapter 5
% +--------------------------------------------------------------------+

\cleardoublepage

% +--------------------------------------------------------------------+
% | Replace "This is Chapter 5" below with the title of your chapter.
% | LaTeX will automatically number the chapters.                      
% +--------------------------------------------------------------------+

\chapter{Appendix}
\label{makereference5}

Here are more examples of references to previous sections.  In Chapter~\ref{makereference5} there were several sections, including section~\ref{makereference5.1}, section~\ref{makereference5.2}, and section~\ref{makereference5.3}.

Likewise, in Chapter~\ref{makereference2}, there are sections~\ref{makereference5.1} and ~\ref{makereference5.2}.





% +--------------------------------------------------------------------+
% | Sample Chapter 4
% +--------------------------------------------------------------------+

\cleardoublepage

% +--------------------------------------------------------------------+
% | Replace "This is Chapter 3" below with the title of your chapter.
% | LaTeX will automatically number the chapters.                      
% +--------------------------------------------------------------------+

%\chapter{Applications}

%\section{Implications for Exceptional Collections}


%Efimov disproved King's conjecture for toric Fano varieties \cite{Efimov2014}.............





% \section{Relationship to HMS}




%\label{makereference4}

%Here are more examples of references to previous sections.  In Chapter~\ref{makereference1} there were several sections, including section~\ref{makereference4.1}, section~\ref{makereference4.2}, and section~\ref{makereference4.3}.

%Likewise, in Chapter~\ref{makereference2}, there are sections~\ref{makereference4.1} and ~\ref{makereference4.2}.


==> nomenclature.tex <==

\nomenclature{$k$}{An algebraically closed field, which can be taken as $k=\C$ throughout.}

\nomenclature{$D^b_{Coh}(X_\Sigma)$}{The bounded derived category of coherent sheaves on the toric variety $X_\Sigma$}

\nomenclature{$S$}{The polynomial ring $S=k[\A^{2n}]=k[x_1,\dots, x_n,y_1, \dots, y_n]$.}

\nomenclature{$\mathcal{F}_{\mathcal{H}_L^\epsilon}^\bullet$}{Cellular resolution of the cellular complex $\mathcal{H}_L^\epsilon$. }

\nomenclature{$\mathcal{H}_L^\epsilon$}{Deformation of the infinite hyperplane arrangement $\mathcal{H}_L$ by the element $\epsilon$ in the effective cone of $X_\Sigma$. Also used to denote the cellular complex given by the intersection of this infinite hyperplane arrangement with $\R L$.  }

\nomenclature{$\mathcal{F}_{\mathcal{H}_L}^\bullet$}{Cellular resolution of the cellular complex $\mathcal{H}_L$. }

\nomenclature{$\mathcal{H}_L$}{The infinite hyperplane arrangement given by all integral shifts of coordinate hyperplanes in $\R^n$, $\{x_i=r \} $ for $r\in \Z$ and $1\leq i \leq n$. Here $n$ denotes the number of primitive ray generators in $\Sigma$.  $\mathcal{H}_L$ is also used to denote the cellular complex given by the intersection of this infinite hyperplane arrangement with $\R L$ }

\nomenclature{$\R L$}{$L \otimes_\Z \R$}

\nomenclature{$L$}{A sublattice of $\Z^n$ for some $n$. For a complete simplicial toric variety $X_\Sigma$ with no torus factors, $L$ denotes the lattice of principal divisors }% given as $\text{Im } B = \ker \pi$ in  \[ 0 \rightarrow \Z^m \stackrel{B}{\rightarrow} \Z^n \stackrel{\pi}{\rightarrow} Cl(X) \rightarrow 0 \] with $\text{rank} M = m$, $n=|\Sigma(1)|$ and $B$ has row vectors given by primitive ray generators in $\Sigma$. }


\nomenclature{$Cl(X_\Sigma)$}{The class group of the toric variety $X_\Sigma$}

\nomenclature{$D_\rho$}{The divisor $x_\rho=0$ corresponding to the ray generator $\rho\in\Sigma(1)$. } 

\nomenclature{$\rho \in \Sigma(1)$}{The one-dimensional cone (also called a ``ray") $\rho$ in the the fan $\Sigma$. At times, we also use $\rho\in \Sigma(1)$ to denote the variable $x_\rho\in S= \C[x_\rho: \rho\in \Sigma(1)]$ in the homogeneous coordinate ring $S$ for $X_\Sigma$, which is graded by the class group of $X_\Sigma$.}


\nomenclature{$\sigma$}{A strongly convex rational polyhedral cone in $N_\R=N \otimes_\Z \R$}


\nomenclature{$X_\Sigma$}{Toric variety $X$ associated to the fan $\Sigma \subset N_\R$}

\nomenclature{M}{The dual lattice $Hom_\Z(N, \Z)$ of characters}

\nomenclature{N}{The lattice of one-parameter subgroups, isomorphic to $\Z^m$ for some $m\in \mathbb{N}$}







